Few Batches or Little Memory, But Not Both: Simultaneous Space and Adaptivity Constraints in Stochastic Bandits

We study stochastic multi-armed bandits under simultaneous constraints on space and adaptivity: the learner interacts with the environment in $B$ batches and has only $W$ bits of persistent memory. Prior work shows that each constraint alone is surprisingly mild: near-minimax regret $\widetilde{O}(\sqrt{KT})$ is achievable with $O(\log T)$ bits of memory under fully adaptive interaction, and with a $K$-independent $O(\log\log T)$-type number of batches when memory is unrestricted. We show that this picture breaks down in the simultaneously constrained regime. We prove that any algorithm with a $W$-bit memory constraint must use at least $\Omega(K/W)$ batches to achieve near-minimax regret $\widetilde{O}(\sqrt{KT})$, even under adaptive grids. In particular, logarithmic memory rules out $O(K^{1-\varepsilon})$ batch complexity. Our proof is based on an information bottleneck. We show that near-minimax regret forces the learner to acquire $\Omega(K)$ bits of information about the hidden set of good arms under a suitable hard prior, whereas an algorithm with $B$ batches and $W$ bits of memory allows only $O(BW)$ bits of information. A key ingredient is a localized change-of-measure lemma that yields probability-level arm exploration guarantees, which is of independent interest. We also give an algorithm that, for any bit budget $W$ with $\Omega(\log T) \le W \le O(K\log T)$, uses at most $W$ bits of memory and $\widetilde{O}(K/W)$ batches while achieving regret $\widetilde{O}(\sqrt{KT})$, nearly matching our lower bound up to polylogarithmic factors.

==> Sections/SubsectionsForFiniteArmLowerbound/lip.tex <==

\section{Hard instances: packing + disjoint tent bumps}


\begin{definition}[Packing number]
For a metric space $(A,d_A)$ and a set $S\subseteq A$, the $r$-packing number $N(S,r)$ is the maximum size
of a packing of $S$ with \emph{disjoint} $d_A$-open balls of radius $r$.
\end{definition}

Fix a radius $\rho\in(0,1)$ and let
\[
    K := N(A,2\rho).
\]
Assume $K$ is even for simplicity.
Then there exist points $\{x_1,\dots,x_K\}\subset A$ such that the open balls
$\{B^\circ(x_i,2\rho)\}_{i=1}^K$ are disjoint.
Hence $d_A(x_i,x_{i'})\ge 4\rho$ for $i\neq i'$ and the closed balls
\[
    \mathcal B_i := \{x\in A: d_A(x,x_i)\le \rho\},\qquad i\in[K],
\]
are pairwise disjoint.

Define the tent profile
\[
    \psi_i(x) := \Big(1-\frac{d_A(x,x_i)}{\rho}\Big)_+ \in [0,1],
\]
which is $(1/\rho)$-Lipschitz and supported on $\mathcal B_i$.
Since the supports are disjoint, for every $x\in A$ we have $\sum_{i=1}^K \psi_i(x)\le 1$.

\paragraph{Instance family.}
Let $\Delta,\Delta_0>0$ satisfy
\begin{equation}\label{eq:amplitude-conditions}
    0<\Delta\le \tfrac{1}{4},\quad 0<\Delta_0\le \tfrac{1}{4},\quad
    \Delta+\Delta_0 \le L\rho.
\end{equation}
Let
\[
    \mathcal U := \{S\subseteq[K]: |S|=K/2\}.
\]
For each $S\in\mathcal U$, define the base mean
\begin{equation}\label{eq:muS}
    \mu_S(x) := \frac{1}{2}-\Delta+\Delta\sum_{i\in S}\psi_i(x),
\end{equation}
and for each $j\in S$, define the perturbed mean
\begin{equation}\label{eq:muS-perturbed}
    \mu_S^{(j)}(x) := \mu_S(x) + \Delta_0 \psi_j(x).
\end{equation}

\begin{lemma}[Validity]\label{lem:validity}
Under \eqref{eq:amplitude-conditions}, we have $\mu_S,\mu_S^{(j)}\in \mathcal F_L$ for all $S\in\mathcal U$ and $j\in S$,
and $\mu_S(x),\mu_S^{(j)}(x)\in[0,1]$ for all $x\in A$.
\end{lemma}

\begin{proof}
First, since $\sum_{i\in S}\psi_i(x)\in[0,1]$, we have
$\mu_S(x)\in[1/2-\Delta,\,1/2] \subseteq [0,1]$ (because $\Delta\le 1/4$).
Similarly, $\mu_S^{(j)}(x)\le 1/2+\Delta_0\le 3/4$ and
$\mu_S^{(j)}(x)\ge 1/2-\Delta\ge 1/4$, so $\mu_S^{(j)}(x)\in[0,1]$.

Second, each $\psi_i$ is $(1/\rho)$-Lipschitz. Using that at every $x$ at most one $\psi_i(x)$ is nonzero
(because the supports $\mathcal B_i$ are disjoint), we have for all $x,x'\in A$,
\[
    \sum_{i\in S} |\psi_i(x)-\psi_i(x')| \le \frac{1}{\rho} d_A(x,x').
\]
Hence
\[
    |\mu_S(x)-\mu_S(x')|
    \le \Delta \sum_{i\in S} |\psi_i(x)-\psi_i(x')|
    \le \frac{\Delta}{\rho} d_A(x,x')
    \le L\, d_A(x,x'),
\]
where the last inequality uses $\Delta\le L\rho$ (implied by $\Delta+\Delta_0\le L\rho$).
For $\mu_S^{(j)}$ we similarly obtain
\[
|\mu_S^{(j)}(x)-\mu_S^{(j)}(x')|
\le \frac{\Delta+\Delta_0}{\rho}d_A(x,x')
\le L\, d_A(x,x'),
\]
where we used $\Delta+\Delta_0\le L\rho$.
\end{proof}


